When can Multi-Site Datasets be Pooled for Regression? Hypothesis Tests, $\ell_2$-consistency and Neuroscience Applications

Many studies in biomedical and health sciences involve small sample sizes due to logistic or financial constraints. Often, identifying weak (but scientifically interesting) associations between a set of predictors and a response necessitates pooling datasets from multiple diverse labs or groups. While there is a rich literature in statistical machine learning to address distributional shifts and inference in multi-site datasets, it is less clear ${\it when}$ such pooling is guaranteed to help (and when it does not) -- independent of the inference algorithms we use. In this paper, we present a hypothesis test to answer this question, both for classical and high dimensional linear regression. We precisely identify regimes where pooling datasets across multiple sites is sensible, and how such policy decisions can be made via simple checks executable on each site before any data transfer ever happens. With a focus on Alzheimer's disease studies, we present empirical results showing that in regimes suggested by our analysis, pooling a local dataset with data from an international study improves power.

==> Relatedwork.tex <==

%% \section{Related Work}
%%  We present related work of hypothesis test, high dimensional setting, and simultaneous inference in the following consecutive paragraphs. 
 
%%  {\bf Hypothesis Test.} For adaptation algorithms, we recommend readers to surveys \cite{patel15},\cite{li12} for a more detailed overview. There have been various literature on theoretical analysis for adaptation algorithms \cite{ben10},\cite{cortes11}. However, they focus on the algorithm itself under specific assumptions, rather than studying whether pooling multiple sites after adaptation is beneficial. A related work to ours is \cite{zhou16}, which tests whether feature distributions match after some types of transformations. However, this work requires the feature distortion assumption, where all differences are assumed to be caused by distortion on features. Our work, which doesn't rely on sampling bias or feature distortion assumptions, tests whether pooling multiple sites after adaptation improves estimation of interesting features. \smallskip

%% {\bf High Dimension.} There has been significant interest in the analysis of multi-task representation learning \cite{maurer16},\cite{ando05},\cite{maurer13}, which assume multiple tasks have same low-dimension representation. In linear regression setting, the analysis is different. Lasso-based models can efficiently find important coefficients. Therefore, the specific structure of Lasso should be taken into account, which leads to the development of multi-task Lasso\cite{liuml09}. However, it still assumes multiple tasks have same active feature set. In practice, tasks might share same properties but also have unique characteristic, such as detecting emotions of children and adults. Therefore, we need a model which allows common properties (across-tasks active) and unique characteristic (task-unique) exists simultaneously. Sparse multi-task Lasso was proposed in \cite{lee10} to explain that. In the original paper, prior information is also used to penalize coefficients, which we'll not discuss here. Sparse multi-task Lasso  has been used in many applications \cite{lee10}\cite{chen12}. However, theoretical analysis and choices of trade-off tuning parameter are hardly known. A highly related work in statistical community is sparse group Lasso \cite{simon13}, which includes multi-task as a special case. In this direction, theory was proposed on $l_2$ consistency \cite{chatterjee12}. However, this work uses general analysis for M-estimators; therefore, it's not informative enough for understanding sparse group Lasso, not to mention sparse multi-task Lasso. We follow the path of analyses for Lasso \cite{mein09} and group Lasso \cite{liugl09}, which have mild assumptions. In sparse multitask Lasso, the block design structure needs to be incorporated and the joint effects of two penalties induces asymmetric structure. We overcome these theoretical difficulty and propose $l_2$ consistency rate. This rate is consistent with Lasso and group Lasso in their favored case. Between two extremes, this rate shows the advantage of sparse multi-task Lasso.

%% {\bf Simultaneous Inference on High Dimension.} The survey \cite{dezeure15} summarizes current progress on high dimensional simultaneous inference, such as multi sample-splitting and de-biased Lasso, and produces an R package hdi for public use. In the survey, thorough simulations are provided to show the effectiveness of  these methods. 

%% Multi sample-splitting method divide samples into two equal halves, where the first half is used for variable selection and the second half with the selected variables are used for calculating p-value; repeat this step several times and calculate adjusted p-value.
%% De-biased Lasso choose one feature as response and the other as predictors, then it fits Lasso for this model; the procedure repeated p times for each feature. Then adjustment for original Lasso solution is made based on these models. De-biased Lasso asymptotically follows normal distribution. It can be used with Bonferroni-Holm adjustment to produce simultaneous p-values. 

%% In our work, we apply high dimensional simultaneous inference to obtain a prior set for important features. In some cases, this prior set is already good enough to select features. In other cases, we use it to help  sparse multi-task Lasso. We show the prior set helps to decide tuning parameter which balances Lasso and group Lasso penalties. 


%De-biased Lasso conducts one-step adjustment after Lasso, and it asymptotically follows normal distribution. Multiple sample-splitting conducts variable selection on one part of data and impose ordinary linear regression test on selected variables using other part of data; the step is repeated several times and adjusted p-values are produced. 

